Kirby belts, categorified projectors, and the skein lasagna module of $S^{2}\times{S^{2}}$

We interpret Manolescu-Neithalath's cabled Khovanov homology formula for computing Morrison-Walker-Wedrich's $\mathrm{KhR}_2$ skein lasagna module as a homotopy colimit (mapping telescope) in a completion of the category of complexes over Bar-Natan's cobordism category. Using categorified projectors, we compute the $\mathrm{KhR}_2$ skein lasagna modules of (manifold, boundary link) pairs $(S^2 \times B^2, \tilde \beta)$, where $\tilde \beta$ is a geometrically essential boundary link, identifying a relationship between the lasagna module and the Rozansky projector appearing in the Rozansky-Willis invariant for nullhomologous links in $S^2 \times S^1$. As an application, we show that the $\mathrm{KhR}_2$ skein lasagna module of $S^2 \times S^2$ is trivial, confirming a conjecture of Manolescu.

==> tikz-imgs/Pn-input.tex <==

% blank strips, vertical strands
\def\g{.3};
\foreach \x in {-2,0,2}{
    \draw (\x,0) -- (\x,2);
    \draw (\x,4) -- (\x,6);
}
\draw (-3,2) rectangle (3,4);
\node at (1,5) {$\cdots$};



==> tikz-imgs/R1-neg-0res-input.tex <==
\draw (0,.5) arc (0:360:.5cm);
\draw (0,-1) .. controls (0, -.1) and (.1, 0) .. (1,0);

==> tikz-imgs/R1-neg-1res-input.tex <==
\draw (0,.5) arc (0:270:.5cm);
\draw (0,.5) .. controls (.1,0) .. (1,0);
\draw (-.5,0) .. controls (0,-.1) .. (0,-1);

==> tikz-imgs/R1-neg-input.tex <==
\draw (-.5,0) -- (1,0);
\fill[white] (0,0) circle (.2cm);
\draw (0,.5) -- (0,-1);
\draw (0,.5) arc (0:270:.5cm);

==> tikz-imgs/R1-neg-reduced-input.tex <==
\draw (0,-1) .. controls (0, -.1) and (.1, 0) .. (1,0);

==> tikz-imgs/Tn-00-input.tex <==

%
% belt loop
\draw (0,0) circle (3cm);
%
% blank strips, vertical strands
\def\g{.3};
\foreach \x in {-2,0,2}{
    \fill[white](\x-\g,0) rectangle (\x+\g,6); 
    \draw (\x,0) -- (\x,6);
}
% vertical strands, below
\foreach \x in {-2,2}{
    \draw (\x,0) -- (\x,-1.5);
    \draw (\x,-3) -- (\x,-6);
}
\draw (0,0) -- (0,-2);
\draw (0,-4) -- (0,-6);
% labels for multiple strands (ellipsis)
\foreach \y in {5,0,-5}{
    \node at (1.1,\y) {$\cdots$};
}
% braces indicating number of strands
% \node at (0,7) {$\overbrace{\phantom{longword}}^n$};
%%%%%%%%%%%%%%%%%%%%
% some resolutions
\foreach \y in {2,-2}{
    \fill[white] (-2,\y) circle (1.5cm);
}
% 00
\begin{comment}
\draw (-2,3.5) .. controls (-2,2.5) 
    and (-1.1,2.8) .. (-.7,2.92);
\draw (-2,.5) .. controls (-2,2) 
    and (-2.5,2) ..  (-2.9,.8);
%
\begin{scope}[yscale=-1]
    \draw (-2,3.5) .. controls (-2,2.5) 
        and (-1.1,2.8) .. (-.7,2.92);
    \draw (-2,.5) .. controls (-2,2) 
        and (-2.5,2) ..  (-2.9,.8);
\end{scope}
\end{comment}
% 10
\begin{comment}
\draw (-2,3.5) .. controls (-2,2.5) 
    and (-2.5,2) ..  (-2.9,.8);
\draw (-2,.5) .. controls (-2,2) 
    and (-1.1,2.8) .. (-.7,2.92);
%
\begin{scope}[yscale=-1]
    \draw (-2,3.5) .. controls (-2,2.5) 
        and (-1.1,2.8) .. (-.7,2.92);
    \draw (-2,.5) .. controls (-2,2) 
        and (-2.5,2) ..  (-2.9,.8);
\end{scope}
\end{comment}
% 01
\begin{comment}
\draw (-2,3.5) .. controls (-2,2.5) 
    and (-1.1,2.8) .. (-.7,2.92);
\draw (-2,.5) .. controls (-2,2) 
    and (-2.5,2) ..  (-2.9,.8);
%
\begin{scope}[yscale=-1]
    \draw (-2,3.5) .. controls (-2,2.5) 
        and (-2.5,2) ..  (-2.9,.8);
    \draw (-2,.5) .. controls (-2,2) 
        and (-1.1,2.8) .. (-.7,2.92);   
\end{scope}
\end{comment}
% 11
% \begin{comment}
\draw (-2,3.5) .. controls (-2,2.5) 
    and (-2.5,2) ..  (-2.9,.8);
\draw (-2,.5) .. controls (-2,2) 
    and (-1.1,2.8) .. (-.7,2.92);
%
\begin{scope}[yscale=-1]
    \draw (-2,3.5) .. controls (-2,2.5) 
        and (-2.5,2) ..  (-2.9,.8);
    \draw (-2,.5) .. controls (-2,2) 
        and (-1.1,2.8) .. (-.7,2.92);  
\end{scope}
% \end{comment}


==> tikz-imgs/Tn-00-small.tex <==

%
% belt loop
\draw (0,0) circle (3cm);
%
% blank strips, vertical strands
\def\g{.3};
\foreach \x in {-2,0,2}{
    \fill[white](\x-\g,0) rectangle (\x+\g,6); 
    \draw (\x,0) -- (\x,6);
}
% vertical strands, below
\foreach \x in {-2,2}{
    \draw (\x,0) -- (\x,-1.5);
    \draw (\x,-3) -- (\x,-6);
}
\draw (0,0) -- (0,-2);
\draw (0,-4) -- (0,-6);
% labels for multiple strands (ellipsis)
\foreach \y in {5,0,-5}{
    \node at (1.1,\y) {\tiny ...};
}
% braces indicating number of strands
% \node at (0,7) {$\overbrace{\phantom{longword}}^n$};
%%%%%%%%%%%%%%%%%%%%
% some resolutions
\foreach \y in {2,-2}{
    \fill[white] (-2,\y) circle (1.5cm);
}
% 00
\begin{comment}
\draw (-2,3.5) .. controls (-2,2.5) 
    and (-1.1,2.8) .. (-.7,2.92);
\draw (-2,.5) .. controls (-2,2) 
    and (-2.5,2) ..  (-2.9,.8);
%
\begin{scope}[yscale=-1]
    \draw (-2,3.5) .. controls (-2,2.5) 
        and (-1.1,2.8) .. (-.7,2.92);
    \draw (-2,.5) .. controls (-2,2) 
        and (-2.5,2) ..  (-2.9,.8);
\end{scope}
\end{comment}
% 10
\begin{comment}
\draw (-2,3.5) .. controls (-2,2.5) 
    and (-2.5,2) ..  (-2.9,.8);
\draw (-2,.5) .. controls (-2,2) 
    and (-1.1,2.8) .. (-.7,2.92);
%
\begin{scope}[yscale=-1]
    \draw (-2,3.5) .. controls (-2,2.5) 
        and (-1.1,2.8) .. (-.7,2.92);
    \draw (-2,.5) .. controls (-2,2) 
        and (-2.5,2) ..  (-2.9,.8);
\end{scope}
\end{comment}
% 01
\begin{comment}
\draw (-2,3.5) .. controls (-2,2.5) 
    and (-1.1,2.8) .. (-.7,2.92);
\draw (-2,.5) .. controls (-2,2) 
    and (-2.5,2) ..  (-2.9,.8);
%
\begin{scope}[yscale=-1]
    \draw (-2,3.5) .. controls (-2,2.5) 
        and (-2.5,2) ..  (-2.9,.8);
    \draw (-2,.5) .. controls (-2,2) 
        and (-1.1,2.8) .. (-.7,2.92);   
\end{scope}
\end{comment}
% 11
% \begin{comment}
\draw (-2,3.5) .. controls (-2,2.5) 
    and (-2.5,2) ..  (-2.9,.8);
\draw (-2,.5) .. controls (-2,2) 
    and (-1.1,2.8) .. (-.7,2.92);
%
\begin{scope}[yscale=-1]
    \draw (-2,3.5) .. controls (-2,2.5) 
        and (-2.5,2) ..  (-2.9,.8);
    \draw (-2,.5) .. controls (-2,2) 
        and (-1.1,2.8) .. (-.7,2.92);  
\end{scope}
% \end{comment}


==> tikz-imgs/Tn-01-input.tex <==

%
% belt loop
\draw (0,0) circle (3cm);
%
% blank strips, vertical strands
\def\g{.3};
\foreach \x in {-2,0,2}{
    \fill[white](\x-\g,0) rectangle (\x+\g,6); 
    \draw (\x,0) -- (\x,6);
}
% vertical strands, below
\foreach \x in {-2,2}{
    \draw (\x,0) -- (\x,-1.5);
    \draw (\x,-3) -- (\x,-6);
}
\draw (0,0) -- (0,-2);
\draw (0,-4) -- (0,-6);
% labels for multiple strands (ellipsis)
\foreach \y in {5,0,-5}{
    \node at (1.1,\y) {$\cdots$};
}
% braces indicating number of strands
% \node at (0,7) {$\overbrace{\phantom{longword}}^n$};
%%%%%%%%%%%%%%%%%%%%
% some resolutions
\foreach \y in {2,-2}{
    \fill[white] (-2,\y) circle (1.5cm);
}
% 00
\begin{comment}
\draw (-2,3.5) .. controls (-2,2.5) 
    and (-1.1,2.8) .. (-.7,2.92);
\draw (-2,.5) .. controls (-2,2) 
    and (-2.5,2) ..  (-2.9,.8);
%
\begin{scope}[yscale=-1]
    \draw (-2,3.5) .. controls (-2,2.5) 
        and (-1.1,2.8) .. (-.7,2.92);
    \draw (-2,.5) .. controls (-2,2) 
        and (-2.5,2) ..  (-2.9,.8);
\end{scope}
\end{comment}
% 10
% \begin{comment}
\draw (-2,3.5) .. controls (-2,2.5) 
    and (-2.5,2) ..  (-2.9,.8);
\draw (-2,.5) .. controls (-2,2) 
    and (-1.1,2.8) .. (-.7,2.92);
%
\begin{scope}[yscale=-1]
    \draw (-2,3.5) .. controls (-2,2.5) 
        and (-1.1,2.8) .. (-.7,2.92);
    \draw (-2,.5) .. controls (-2,2) 
        and (-2.5,2) ..  (-2.9,.8);
\end{scope}
% \end{comment}
% 01
\begin{comment}
\draw (-2,3.5) .. controls (-2,2.5) 
    and (-1.1,2.8) .. (-.7,2.92);
\draw (-2,.5) .. controls (-2,2) 
    and (-2.5,2) ..  (-2.9,.8);
%
\begin{scope}[yscale=-1]
    \draw (-2,3.5) .. controls (-2,2.5) 
        and (-2.5,2) ..  (-2.9,.8);
    \draw (-2,.5) .. controls (-2,2) 
        and (-1.1,2.8) .. (-.7,2.92);   
\end{scope}
\end{comment}
% 11
\begin{comment}
\draw (-2,3.5) .. controls (-2,2.5) 
    and (-2.5,2) ..  (-2.9,.8);
\draw (-2,.5) .. controls (-2,2) 
    and (-1.1,2.8) .. (-.7,2.92);
%
\begin{scope}[yscale=-1]
    \draw (-2,3.5) .. controls (-2,2.5) 
        and (-2.5,2) ..  (-2.9,.8);
    \draw (-2,.5) .. controls (-2,2) 
        and (-1.1,2.8) .. (-.7,2.92);  
\end{scope}
\end{comment}

==> tikz-imgs/Tn-01-small.tex <==

%
% belt loop
\draw (0,0) circle (3cm);
%
% blank strips, vertical strands
\def\g{.3};
\foreach \x in {-2,0,2}{
    \fill[white](\x-\g,0) rectangle (\x+\g,6); 
    \draw (\x,0) -- (\x,6);
}
% vertical strands, below
\foreach \x in {-2,2}{
    \draw (\x,0) -- (\x,-1.5);
    \draw (\x,-3) -- (\x,-6);
}
\draw (0,0) -- (0,-2);
\draw (0,-4) -- (0,-6);
% labels for multiple strands (ellipsis)
\foreach \y in {5,0,-5}{
    \node at (1.1,\y) {\tiny ...};
}
% braces indicating number of strands
% \node at (0,7) {$\overbrace{\phantom{longword}}^n$};
%%%%%%%%%%%%%%%%%%%%
% some resolutions
\foreach \y in {2,-2}{
    \fill[white] (-2,\y) circle (1.5cm);
}
% 00
\begin{comment}
\draw (-2,3.5) .. controls (-2,2.5) 
    and (-1.1,2.8) .. (-.7,2.92);
\draw (-2,.5) .. controls (-2,2) 
    and (-2.5,2) ..  (-2.9,.8);
%
\begin{scope}[yscale=-1]
    \draw (-2,3.5) .. controls (-2,2.5) 
        and (-1.1,2.8) .. (-.7,2.92);
    \draw (-2,.5) .. controls (-2,2) 
        and (-2.5,2) ..  (-2.9,.8);
\end{scope}
\end{comment}
% 10
% \begin{comment}
\draw (-2,3.5) .. controls (-2,2.5) 
    and (-2.5,2) ..  (-2.9,.8);
\draw (-2,.5) .. controls (-2,2) 
    and (-1.1,2.8) .. (-.7,2.92);
%
\begin{scope}[yscale=-1]
    \draw (-2,3.5) .. controls (-2,2.5) 
        and (-1.1,2.8) .. (-.7,2.92);
    \draw (-2,.5) .. controls (-2,2) 
        and (-2.5,2) ..  (-2.9,.8);
\end{scope}
% \end{comment}
% 01
\begin{comment}
\draw (-2,3.5) .. controls (-2,2.5) 
    and (-1.1,2.8) .. (-.7,2.92);
\draw (-2,.5) .. controls (-2,2) 
    and (-2.5,2) ..  (-2.9,.8);
%
\begin{scope}[yscale=-1]
    \draw (-2,3.5) .. controls (-2,2.5) 
        and (-2.5,2) ..  (-2.9,.8);
    \draw (-2,.5) .. controls (-2,2) 
        and (-1.1,2.8) .. (-.7,2.92);   
\end{scope}
\end{comment}
% 11
\begin{comment}
\draw (-2,3.5) .. controls (-2,2.5) 
    and (-2.5,2) ..  (-2.9,.8);
\draw (-2,.5) .. controls (-2,2) 
    and (-1.1,2.8) .. (-.7,2.92);
%
\begin{scope}[yscale=-1]
    \draw (-2,3.5) .. controls (-2,2.5) 
        and (-2.5,2) ..  (-2.9,.8);
    \draw (-2,.5) .. controls (-2,2) 
        and (-1.1,2.8) .. (-.7,2.92);  
\end{scope}
\end{comment}

==> tikz-imgs/Tn-0s-input.tex <==
%
% belt loop
\draw (0,0) circle (3cm);
%
% blank strips, vertical strands
\def\g{.3};
\foreach \x in {-2,0,2}{
    \fill[white](\x-\g,0) rectangle (\x+\g,6); 
    \draw (\x,0) -- (\x,6);
}
% vertical strands, below
\foreach \x in {-2,2}{
    \draw (\x,0) -- (\x,-1.5);
    \draw (\x,-3) -- (\x,-6);
}
\draw (0,0) -- (0,-2);
\draw (0,-4) -- (0,-6);
% labels for multiple strands (ellipsis)
\foreach \y in {5,0,-5}{
    \node at (1.1,\y) {$\cdots$};
}
% braces indicating number of strands
% \node at (0,7) {$\overbrace{\phantom{longword}}^n$};
%%%%%%%%%%%%%%%%%%%%
% some resolutions
\foreach \y in {2}{
    \fill[white] (-2,\y) circle (1.5cm);
}
% 00
%\begin{comment}
\draw (-2,3.5) .. controls (-2,2.5) 
    and (-1.1,2.8) .. (-.7,2.92);
\draw (-2,.5) .. controls (-2,2) 
    and (-2.5,2) ..  (-2.9,.8);
%
\begin{comment}
\begin{scope}[yscale=-1]
    \draw (-2,3.5) .. controls (-2,2.5) 
        and (-1.1,2.8) .. (-.7,2.92);
    \draw (-2,.5) .. controls (-2,2) 
        and (-2.5,2) ..  (-2.9,.8);
\end{scope}
\end{comment}
% 10
\begin{comment}
\draw (-2,3.5) .. controls (-2,2.5) 
    and (-2.5,2) ..  (-2.9,.8);
\draw (-2,.5) .. controls (-2,2) 
    and (-1.1,2.8) .. (-.7,2.92);
%
\begin{scope}[yscale=-1]
    \draw (-2,3.5) .. controls (-2,2.5) 
        and (-1.1,2.8) .. (-.7,2.92);
    \draw (-2,.5) .. controls (-2,2) 
        and (-2.5,2) ..  (-2.9,.8);
\end{scope}
\end{comment}
% 01
\begin{comment}
\draw (-2,3.5) .. controls (-2,2.5) 
    and (-1.1,2.8) .. (-.7,2.92);
\draw (-2,.5) .. controls (-2,2) 
    and (-2.5,2) ..  (-2.9,.8);
%
\begin{scope}[yscale=-1]
    \draw (-2,3.5) .. controls (-2,2.5) 
        and (-2.5,2) ..  (-2.9,.8);
    \draw (-2,.5) .. controls (-2,2) 
        and (-1.1,2.8) .. (-.7,2.92);   
\end{scope}
\end{comment}
% 11
\begin{comment}
\draw (-2,3.5) .. controls (-2,2.5) 
    and (-2.5,2) ..  (-2.9,.8);
\draw (-2,.5) .. controls (-2,2) 
    and (-1.1,2.8) .. (-.7,2.92);
%
\begin{scope}[yscale=-1]
    \draw (-2,3.5) .. controls (-2,2.5) 
        and (-2.5,2) ..  (-2.9,.8);
    \draw (-2,.5) .. controls (-2,2) 
        and (-1.1,2.8) .. (-.7,2.92);  
\end{scope}
\end{comment}


==> tikz-imgs/Tn-10-input.tex <==

%
% belt loop
\draw (0,0) circle (3cm);
%
% blank strips, vertical strands
\def\g{.3};
\foreach \x in {-2,0,2}{
    \fill[white](\x-\g,0) rectangle (\x+\g,6); 
    \draw (\x,0) -- (\x,6);
}
% vertical strands, below
\foreach \x in {-2,2}{
    \draw (\x,0) -- (\x,-1.5);
    \draw (\x,-3) -- (\x,-6);
}
\draw (0,0) -- (0,-2);
\draw (0,-4) -- (0,-6);
% labels for multiple strands (ellipsis)
\foreach \y in {5,0,-5}{
    \node at (1.1,\y) {$\cdots$};
}
% braces indicating number of strands
% \node at (0,7) {$\overbrace{\phantom{longword}}^n$};
%%%%%%%%%%%%%%%%%%%%
% some resolutions
\foreach \y in {2,-2}{
    \fill[white] (-2,\y) circle (1.5cm);
}
% 00
\begin{comment}
\draw (-2,3.5) .. controls (-2,2.5) 
    and (-1.1,2.8) .. (-.7,2.92);
\draw (-2,.5) .. controls (-2,2) 
    and (-2.5,2) ..  (-2.9,.8);
%
\begin{scope}[yscale=-1]
    \draw (-2,3.5) .. controls (-2,2.5) 
        and (-1.1,2.8) .. (-.7,2.92);
    \draw (-2,.5) .. controls (-2,2) 
        and (-2.5,2) ..  (-2.9,.8);
\end{scope}
\end{comment}
% 10
\begin{comment}
\draw (-2,3.5) .. controls (-2,2.5) 
    and (-2.5,2) ..  (-2.9,.8);
\draw (-2,.5) .. controls (-2,2) 
    and (-1.1,2.8) .. (-.7,2.92);
%
\begin{scope}[yscale=-1]
    \draw (-2,3.5) .. controls (-2,2.5) 
        and (-1.1,2.8) .. (-.7,2.92);
    \draw (-2,.5) .. controls (-2,2) 
        and (-2.5,2) ..  (-2.9,.8);
\end{scope}
\end{comment}
% 01
% \begin{comment}
\draw (-2,3.5) .. controls (-2,2.5) 
    and (-1.1,2.8) .. (-.7,2.92);
\draw (-2,.5) .. controls (-2,2) 
    and (-2.5,2) ..  (-2.9,.8);
%
\begin{scope}[yscale=-1]
    \draw (-2,3.5) .. controls (-2,2.5) 
        and (-2.5,2) ..  (-2.9,.8);
    \draw (-2,.5) .. controls (-2,2) 
        and (-1.1,2.8) .. (-.7,2.92);   
\end{scope}
% \end{comment}
% 11
\begin{comment}
\draw (-2,3.5) .. controls (-2,2.5) 
    and (-2.5,2) ..  (-2.9,.8);
\draw (-2,.5) .. controls (-2,2) 
    and (-1.1,2.8) .. (-.7,2.92);
%
\begin{scope}[yscale=-1]
    \draw (-2,3.5) .. controls (-2,2.5) 
        and (-2.5,2) ..  (-2.9,.8);
    \draw (-2,.5) .. controls (-2,2) 
        and (-1.1,2.8) .. (-.7,2.92);  
\end{scope}
\end{comment}

==> tikz-imgs/Tn-10-small.tex <==

%
% belt loop
\draw (0,0) circle (3cm);
%
% blank strips, vertical strands
\def\g{.3};
\foreach \x in {-2,0,2}{
    \fill[white](\x-\g,0) rectangle (\x+\g,6); 
    \draw (\x,0) -- (\x,6);
}
% vertical strands, below
\foreach \x in {-2,2}{
    \draw (\x,0) -- (\x,-1.5);
    \draw (\x,-3) -- (\x,-6);
}
\draw (0,0) -- (0,-2);
\draw (0,-4) -- (0,-6);
% labels for multiple strands (ellipsis)
\foreach \y in {5,0,-5}{
    \node at (1.1,\y) {\tiny ...};
}
% braces indicating number of strands
% \node at (0,7) {$\overbrace{\phantom{longword}}^n$};
%%%%%%%%%%%%%%%%%%%%
% some resolutions
\foreach \y in {2,-2}{
    \fill[white] (-2,\y) circle (1.5cm);
}
% 00
\begin{comment}
\draw (-2,3.5) .. controls (-2,2.5) 
    and (-1.1,2.8) .. (-.7,2.92);
\draw (-2,.5) .. controls (-2,2) 
    and (-2.5,2) ..  (-2.9,.8);
%
\begin{scope}[yscale=-1]
    \draw (-2,3.5) .. controls (-2,2.5) 
        and (-1.1,2.8) .. (-.7,2.92);
    \draw (-2,.5) .. controls (-2,2) 
        and (-2.5,2) ..  (-2.9,.8);
\end{scope}
\end{comment}
% 10
\begin{comment}
\draw (-2,3.5) .. controls (-2,2.5) 
    and (-2.5,2) ..  (-2.9,.8);
\draw (-2,.5) .. controls (-2,2) 
    and (-1.1,2.8) .. (-.7,2.92);
%
\begin{scope}[yscale=-1]
    \draw (-2,3.5) .. controls (-2,2.5) 
        and (-1.1,2.8) .. (-.7,2.92);
    \draw (-2,.5) .. controls (-2,2) 
        and (-2.5,2) ..  (-2.9,.8);
\end{scope}
\end{comment}
% 01
% \begin{comment}
\draw (-2,3.5) .. controls (-2,2.5) 
    and (-1.1,2.8) .. (-.7,2.92);
\draw (-2,.5) .. controls (-2,2) 
    and (-2.5,2) ..  (-2.9,.8);
%
\begin{scope}[yscale=-1]
    \draw (-2,3.5) .. controls (-2,2.5) 
        and (-2.5,2) ..  (-2.9,.8);
    \draw (-2,.5) .. controls (-2,2) 
        and (-1.1,2.8) .. (-.7,2.92);   
\end{scope}
% \end{comment}
% 11
\begin{comment}
\draw (-2,3.5) .. controls (-2,2.5) 
    and (-2.5,2) ..  (-2.9,.8);
\draw (-2,.5) .. controls (-2,2) 
    and (-1.1,2.8) .. (-.7,2.92);
%
\begin{scope}[yscale=-1]
    \draw (-2,3.5) .. controls (-2,2.5) 
        and (-2.5,2) ..  (-2.9,.8);
    \draw (-2,.5) .. controls (-2,2) 
        and (-1.1,2.8) .. (-.7,2.92);  
\end{scope}
\end{comment}

==> tikz-imgs/Tn-11-input.tex <==
%
% belt loop
\draw (0,0) circle (3cm);
%
% blank strips, vertical strands
\def\g{.3};
\foreach \x in {-2,0,2}{
    \fill[white](\x-\g,0) rectangle (\x+\g,6); 
    \draw (\x,0) -- (\x,6);
}
% vertical strands, below
\foreach \x in {-2,2}{
    \draw (\x,0) -- (\x,-1.5);
    \draw (\x,-3) -- (\x,-6);
}
\draw (0,0) -- (0,-2);
\draw (0,-4) -- (0,-6);
% labels for multiple strands (ellipsis)
\foreach \y in {5,0,-5}{
    \node at (1.1,\y) {$\cdots$};
}
% braces indicating number of strands
% \node at (0,7) {$\overbrace{\phantom{longword}}^n$};
%%%%%%%%%%%%%%%%%%%%
% some resolutions
\foreach \y in {2,-2}{
    \fill[white] (-2,\y) circle (1.5cm);
}
% 00
% \begin{comment}
\draw (-2,3.5) .. controls (-2,2.5) 
    and (-1.1,2.8) .. (-.7,2.92);
\draw (-2,.5) .. controls (-2,2) 
    and (-2.5,2) ..  (-2.9,.8);
%
\begin{scope}[yscale=-1]
    \draw (-2,3.5) .. controls (-2,2.5) 
        and (-1.1,2.8) .. (-.7,2.92);
    \draw (-2,.5) .. controls (-2,2) 
        and (-2.5,2) ..  (-2.9,.8);
\end{scope}
% \end{comment}
% 10
\begin{comment}
\draw (-2,3.5) .. controls (-2,2.5) 
    and (-2.5,2) ..  (-2.9,.8);
\draw (-2,.5) .. controls (-2,2) 
    and (-1.1,2.8) .. (-.7,2.92);
%
\begin{scope}[yscale=-1]
    \draw (-2,3.5) .. controls (-2,2.5) 
        and (-1.1,2.8) .. (-.7,2.92);
    \draw (-2,.5) .. controls (-2,2) 
        and (-2.5,2) ..  (-2.9,.8);
\end{scope}
\end{comment}
% 01
\begin{comment}
\draw (-2,3.5) .. controls (-2,2.5) 
    and (-1.1,2.8) .. (-.7,2.92);
\draw (-2,.5) .. controls (-2,2) 
    and (-2.5,2) ..  (-2.9,.8);
%
\begin{scope}[yscale=-1]
    \draw (-2,3.5) .. controls (-2,2.5) 
        and (-2.5,2) ..  (-2.9,.8);
    \draw (-2,.5) .. controls (-2,2) 
        and (-1.1,2.8) .. (-.7,2.92);   
\end{scope}
\end{comment}
% 11
\begin{comment}
\draw (-2,3.5) .. controls (-2,2.5) 
    and (-2.5,2) ..  (-2.9,.8);
\draw (-2,.5) .. controls (-2,2) 
    and (-1.1,2.8) .. (-.7,2.92);
%
\begin{scope}[yscale=-1]
    \draw (-2,3.5) .. controls (-2,2.5) 
        and (-2.5,2) ..  (-2.9,.8);
    \draw (-2,.5) .. controls (-2,2) 
        and (-1.1,2.8) .. (-.7,2.92);  
\end{scope}
\end{comment}


==> tikz-imgs/Tn-11-small.tex <==
%
% belt loop
\draw (0,0) circle (3cm);
%
% blank strips, vertical strands
\def\g{.3};
\foreach \x in {-2,0,2}{
    \fill[white](\x-\g,0) rectangle (\x+\g,6); 
    \draw (\x,0) -- (\x,6);
}
% vertical strands, below
\foreach \x in {-2,2}{
    \draw (\x,0) -- (\x,-1.5);
    \draw (\x,-3) -- (\x,-6);
}
\draw (0,0) -- (0,-2);
\draw (0,-4) -- (0,-6);
% labels for multiple strands (ellipsis)
\foreach \y in {5,0,-5}{
    \node at (1.1,\y) {{\tiny ...}};
}
% braces indicating number of strands
% \node at (0,7) {$\overbrace{\phantom{longword}}^n$};
%%%%%%%%%%%%%%%%%%%%
% some resolutions
\foreach \y in {2,-2}{
    \fill[white] (-2,\y) circle (1.5cm);
}
% 00
% \begin{comment}
\draw (-2,3.5) .. controls (-2,2.5) 
    and (-1.1,2.8) .. (-.7,2.92);
\draw (-2,.5) .. controls (-2,2) 
    and (-2.5,2) ..  (-2.9,.8);
%
\begin{scope}[yscale=-1]
    \draw (-2,3.5) .. controls (-2,2.5) 
        and (-1.1,2.8) .. (-.7,2.92);
    \draw (-2,.5) .. controls (-2,2) 
        and (-2.5,2) ..  (-2.9,.8);
\end{scope}
% \end{comment}

==> tikz-imgs/Tn-1s-input.tex <==
%
% belt loop
\draw (0,0) circle (3cm);
%
% blank strips, vertical strands
\def\g{.3};
\foreach \x in {-2,0,2}{
    \fill[white](\x-\g,0) rectangle (\x+\g,6); 
    \draw (\x,0) -- (\x,6);
}
% vertical strands, below
\foreach \x in {-2,2}{
    \draw (\x,0) -- (\x,-1.5);
    \draw (\x,-3) -- (\x,-6);
}
\draw (0,0) -- (0,-2);
\draw (0,-4) -- (0,-6);
% labels for multiple strands (ellipsis)
\foreach \y in {5,0,-5}{
    \node at (1.1,\y) {$\cdots$};
}
% braces indicating number of strands
% \node at (0,7) {$\overbrace{\phantom{longword}}^n$};
%%%%%%%%%%%%%%%%%%%%
% some resolutions
\foreach \y in {2}{
    \fill[white] (-2,\y) circle (1.5cm);
}
% 00
\begin{comment}
\draw (-2,3.5) .. controls (-2,2.5) 
    and (-1.1,2.8) .. (-.7,2.92);
\draw (-2,.5) .. controls (-2,2) 
    and (-2.5,2) ..  (-2.9,.8);
%
\begin{scope}[yscale=-1]
    \draw (-2,3.5) .. controls (-2,2.5) 
        and (-1.1,2.8) .. (-.7,2.92);
    \draw (-2,.5) .. controls (-2,2) 
        and (-2.5,2) ..  (-2.9,.8);
\end{scope}
\end{comment}
% 10
% \begin{comment}
\draw (-2,3.5) .. controls (-2,2.5) 
    and (-2.5,2) ..  (-2.9,.8);
\draw (-2,.5) .. controls (-2,2) 
    and (-1.1,2.8) .. (-.7,2.92);
%
\begin{comment}
\begin{scope}[yscale=-1]
    \draw (-2,3.5) .. controls (-2,2.5) 
        and (-1.1,2.8) .. (-.7,2.92);
    \draw (-2,.5) .. controls (-2,2) 
        and (-2.5,2) ..  (-2.9,.8);
\end{scope}
\end{comment}
% 01
\begin{comment}
\draw (-2,3.5) .. controls (-2,2.5) 
    and (-1.1,2.8) .. (-.7,2.92);
\draw (-2,.5) .. controls (-2,2) 
    and (-2.5,2) ..  (-2.9,.8);
%
\begin{scope}[yscale=-1]
    \draw (-2,3.5) .. controls (-2,2.5) 
        and (-2.5,2) ..  (-2.9,.8);
    \draw (-2,.5) .. controls (-2,2) 
        and (-1.1,2.8) .. (-.7,2.92);   
\end{scope}
\end{comment}
% 11
\begin{comment}
\draw (-2,3.5) .. controls (-2,2.5) 
    and (-2.5,2) ..  (-2.9,.8);
\draw (-2,.5) .. controls (-2,2) 
    and (-1.1,2.8) .. (-.7,2.92);
%
\begin{scope}[yscale=-1]
    \draw (-2,3.5) .. controls (-2,2.5) 
        and (-2.5,2) ..  (-2.9,.8);
    \draw (-2,.5) .. controls (-2,2) 
        and (-1.1,2.8) .. (-.7,2.92);  
\end{scope}
\end{comment}


==> tikz-imgs/Tn-input-braces.tex <==
%
% belt loop
\draw (0,0) circle (3cm);
%
% blank strips, vertical strands
\def\g{.3};
\foreach \x in {-2,0,2}{
    \fill[white](\x-\g,0) rectangle (\x+\g,6); 
    \draw (\x,0) -- (\x,6);
}
% vertical strands, below
\foreach \x in {-2,2}{
    \draw (\x,0) -- (\x,-1.5);
    \draw (\x,-3) -- (\x,-6);
}
\draw (0,0) -- (0,-2);
\draw (0,-4) -- (0,-6);
% labels for multiple strands (ellipsis)
\foreach \y in {5,0,-5}{
    \node at (1.1,\y) {$\cdots$};
}
% braces indicating number of strands
\node at (0,7) {$\overbrace{\phantom{longword}}^n$};



==> tikz-imgs/Tn-input.tex <==
%
% belt loop
\draw (0,0) circle (3cm);
%
% blank strips, vertical strands
\def\g{.3};
\foreach \x in {-2,0,2}{
    \fill[white](\x-\g,0) rectangle (\x+\g,6); 
    \draw (\x,0) -- (\x,6);
}
% vertical strands, below
\foreach \x in {-2,2}{
    \draw (\x,0) -- (\x,-1.5);
    \draw (\x,-3) -- (\x,-6);
}
\draw (0,0) -- (0,-2);
\draw (0,-4) -- (0,-6);
% labels for multiple strands (ellipsis)
\foreach \y in {5,0,-5}{
    \node at (1.1,\y) {$\cdots$};
}
% braces indicating number of strands
% \node at (0,7) {$\overbrace{\phantom{longword}}^n$};



==> tikz-imgs/ori-input.tex <==
\begin{scope}[xshift=-.5cm, yshift=-.5cm]
\draw[->] (0,0) .. controls (.5, .5).. (0,1);
\draw[->] (1,0) .. controls (.5, .5).. (1,1);
\end{scope}
